InvGC: Robust Cross-Modal Retrieval by Inverse Graph Convolution

Over recent decades, significant advancements in cross-modal retrieval are mainly driven by breakthroughs in visual and linguistic modeling. However, a recent study shows that multi-modal data representations tend to cluster within a limited convex cone (as representation degeneration problem), which hinders retrieval performance due to the inseparability of these representations. In our study, we first empirically validate the presence of the representation degeneration problem across multiple cross-modal benchmarks and methods. Next, to address it, we introduce a novel method, called InvGC, a post-processing technique inspired by graph convolution and average pooling. Specifically, InvGC defines the graph topology within the datasets and then applies graph convolution in a subtractive manner. This method effectively separates representations by increasing the distances between data points. To improve the efficiency and effectiveness of InvGC, we propose an advanced graph topology, LocalAdj, which only aims to increase the distances between each data point and its nearest neighbors. To understand why InvGC works, we present a detailed theoretical analysis, proving that the lower bound of recall will be improved after deploying InvGC. Extensive empirical results show that InvGC and InvGC w/LocalAdj significantly mitigate the representation degeneration problem, thereby enhancing retrieval performance. Our code is available at https://github.com/yimuwangcs/Better_Cross_Modal_Retrieval

==> utils.tex <==
% \usepackage{graphicx}
% \usepackage{enumerate}
% \usepackage{extarrows}              %实现长等号等
% \usepackage{amssymb}                      % AMSLaTeX宏包 用来排出更加漂亮的公式
% \usepackage{amsmath}
% \usepackage{mathrsfs}                     % 不同于\mathcal or \mathfrak 之类的英文花体字体
% \allowdisplaybreaks % 允许公式跨页显示
% \usepackage{bm}                           % 处理数学公式中的黑斜体的宏包
% \usepackage[amsmath,thmmarks]{ntheorem}  % 定理类环境宏包，其中 amsmath 选项用来兼容 AMS LaTeX 的宏包thmmarks 选项，可以自动恰当地放置定理类环境的结束标记；它还能像图形目录那样生成定理类环境目录
% \usepackage{amsfonts}
\usepackage{colortbl}
%\usepackage[table,dvipsnames]{xcolor}
\usepackage{wrapfig}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{microtype}
\usepackage{fixltx2e}
\usepackage{comment}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{booktabs} % To thicken table lines
\usepackage{pifont}
% \usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
% \usepackage{amsopn}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{amsfonts}
% \usepackage{booktabs}
\usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{natbib}
% \usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amsthm}
\usepackage{nameref}

\usepackage{subfig}
\usepackage{subfloat}
% \usepackage{caption}
% \usepackage{subcaption}

\usepackage[american]{babel}

\usepackage{color}

\usepackage{graphicx}
\allowdisplaybreaks


% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}

% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\onedot{.}
\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} 
\def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

\def \wlogs {\emph{w.l.o.g}\onedot}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\bnl}{Bernoulli}
\DeclareMathOperator*{\indicator}{\mathbf{1}}
% \DeclareMathOperator*{\inf}{inf}
% \DeclareMathOperator*{\sup}{sup}

\def \expectation {\mathbf{E}}

\def \domX {\mathcal{X}}
\def \domF {\mathcal{F}}






% \def \D {\mathcal{D}}



% % \def \t {t}
% % \def \T {T}
% \def \Clip {\mathop{\text{Clip}}}
% \def \tree {\mathop{\text{CTB}}}

% \def \m {\bm{m}}

% \def \R {R}
% \def \d {d}

% \def \f {f}
% \def \x {\bm{x}}
% \def \X {\mathcal{X}}
% \def \y {\bm{y}}
% \def \g {\bm{g}}
% \def \G {\mathbf{G}}
% \def \H {\mathbf{H}}
% \def \s {\bm{s}}
% \def \S {\mathbf{S}}

% \def \z {\bm{z}}

% \def \I {\mathbf{I}}
% \def \diag {\operatorname{diag}}

% \def \ng {\tilde{\g}}
% \def \nG {\tilde{\G}}
% \def \ns {\tilde{\s}}
% \def \nS {\tilde{\S}}
% % \def \nSc {\tilde{\S}^{\dag}}
% \def \nGc {\tilde{\G}^{\dag}}
% \def \nH {\tilde{\H}}

% \def \n {\bm{n}}
% \def \N {\mathbf{N}}

% \def \B {B}
% \def \tB {\tilde{\B}}
% \def \i {i}

% \def \RR {\operatorname{RandomizedResponse}}

% \def \M {\mathcal{M}}
% \def \estimate {\mathbb{E}}

% \def \SR {\mathbb{R}}
% \def \SS {\mathcal{S}}

% \def \vz {\bm{0}}
% \def \vo {\bm{1}}

% \def \n {\bm{n}}
% \def \N {\N}

% \def \D {D}
% \def \G {G}

% \def \X {\mathcal{X}}
% \def \x {\bm{x}}

% \def \t {t}
% \def \T {T}
% \def \d {d}

% \def \g {\bm{g}}

% \def \F {\mathcal{F}}
% \def \f {f}

% \def \m {\bm{m}}
% \def \hm {\hat{\m}}

% \def \v {\bm{v}}
% \def \V {V}
% \def \hv {\hat{\v}}
% \def \hV {\hat{\V}}

% \def \diag {\mbox{diag}}


% \def \u {\bm{u}}
% \def \z {\bm{z}}

% \def \Z {Z}


% \def \i {i}
% \def \j {j}
% \def \k {k}
% \def \y {y}

% \def \R {R}



\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}

\newtheorem{condition}{Condition}

\newtheorem{remark}{Remark}

% \newtheorem{lemma}{Lemma}
% \newtheorem{example}{Example}
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}

% \renewcommand{\algorithmicrequire}{\textbf{~Input:}}
% \renewcommand{\algorithmicensure}{\textbf{~Output:}}
% \renewcommand{\algorithmiccomment}[1]{// #1}

% % 重定义某些数学符号，方便使用
% \newcommand{\argmax}{\mathop{\arg\max}}
% \newcommand{\argmin}{\mathop{\arg\min}}
% \newcommand{\med}{\mathop{\textrm{med}}}
% \newcommand{\expect}{\mathbb{E}}
% \newcommand{\sign}{\mathop{\text{sign}}}
% \newcommand{\mathI}{\mathcal{I}}



\DeclareMathOperator*{\tr}{trace}
% \DeclareMathOperator*{\rk}{rank}
% \DeclareMathOperator*{\st}{s.t.}
% \DeclareMathOperator*{\pr}{Pr}
% \DeclareMathOperator*{\vr}{Var}
% \DeclareMathOperator*{\sgn}{sign}
% \DeclareMathOperator*{\dom}{dom}

\newcounter{mylabelcounter}

\makeatletter
\newcommand{\labelText}[2]{%
#1\refstepcounter{mylabelcounter}%
\immediate\write\@auxout{%
  \string\newlabel{#2}{{1}{\thepage}{{\unexpanded{#1}}}{mylabelcounter.\number\value{mylabelcounter}}{}}%
}%
}
\makeatother

% \DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\argmin}{argmin}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\g}{\mathbf{g}}
\renewcommand{\u}{\bm{u}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\w}{\bm{w}}
\newcommand{\x}{\bm{x}}
\newcommand{\y}{\bm{y}}
\newcommand{\bo}{\bm{o}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\K}{\mathcal{K}}
\renewcommand{\L}{\mathbf{L}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\N}{\mathcal{N}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\rank}{\textup{\textsf{rank}}}
\newcommand{\orthc}{\mathbf{orth}_c}
\newcommand{\orthr}{\mathbf{orth}_r}
\newcommand{\bLambda}{\mathbf{\Lambda}}
\newcommand{\RS}{\mathcal{R}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}
\renewcommand{\comment}[1]{}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
% \newcommand{\tr}{\textsf{tr}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbI}{\mathbb{I}}
% \newcommand{\Pr}{\mathbb{P}}
\newcommand{\Pro}{\text{Pro}}
\newcommand{\spann}{\textsf{span}}
\newcommand{\dist}{\textup{\textrm{dist}}}
\newcommand{\erf}{\textup{\textrm{erf}}}
\newcommand{\vol}{\textsf{vol}}
\newcommand{\Null}{\textsf{null}}
\newcommand{\Area}{\textsf{Area}}

% \DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\argmin}{argmin}

\newlength\myindent % define a new length \myindent
\setlength\myindent{6em} % assign the length 2em to \myindet
\newcommand\bindent{%
  \begingroup % starts a group (to keep changes local)
  \setlength{\itemindent}{\myindent} % set itemindent (algorithmic internally uses a list) to the value of \mylength
  \addtolength{\algorithmicindent}{\myindent} % adds \mylength to the default indentation used by algorithmic
}
\newcommand\eindent{\endgroup} % closes a group

\algdef{SE}[SUBALG]{Indent}{EndIndent}{}{\algorithmicend\ }%
\algtext*{Indent}
\algtext*{EndIndent}

